From formal smoothings to geometric smoothings

Let X be a projective, equidimensional, singular scheme over an algebraically closed field. Then the existence of a geometric smoothing (i.e. a family of deformations of X over a smooth base curve whose generic fibre is smooth) implies the existence of a formal smoothing as defined by Tziolas. In this paper we address the reverse question giving sufficient conditions on X that guarantee the converse, i.e. formal smoothability implies geometric smoothability. This is useful in light of Tziolas' results giving sufficient criteria for the existence of formal smoothings.

==> bibliography.tex <==
@misc{stacks-project,
    shorthand    = {Stacks},
    author       = {The {Stacks Project Authors}},
    title        = {\textit{Stacks Project}},
    howpublished = {\url{https://stacks.math.columbia.edu}},
    year         = {2018},
  }
  
@article{MR0217083,
	shorthand = {EGA1},
	Author = {Grothendieck, A. and Dieudonn{\'e}, J. A.},
	Date-Added = {2018-03-24 22:13:35 +0000},
	Date-Modified = {2018-03-24 22:13:35 +0000},
	Fjournal = {Institut des Hautes {\'E}tudes Scientifiques. Publications Math{\'e}matiques},
	Issn = {0073-8301},
	Journal = {Inst. Hautes {\'E}tudes Sci. Publ. Math.},
	Mrclass = {14.55},
	Mrnumber = {0217083},
	Number = {4},
	Pages = {228},
	Title = {{\'E}l{\'e}ments de g{\'e}om{\'e}trie alg{\'e}brique. {I}. {L}e langage des sch{\'e}mas},
	Url = {http://www.numdam.org/item/?id=PMIHES_1960__4__5_0},
	Year = {1960},
	Bdsk-Url-1 = {http://mathscinet.ams.org/mathscinet-getitem?mr=0217083}}

@article{MR0163909,
	Author = {Grothendieck, A. and Dieudonn{\'e}, J. A.},
	Date-Added = {2018-03-24 22:13:24 +0000},
	Date-Modified = {2018-03-24 22:13:24 +0000},
	Fjournal = {Institut des Hautes {\'E}tudes Scientifiques. Publications Math{\'e}matiques},
	Issn = {0073-8301},
	Journal = {Inst. Hautes {\'E}tudes Sci. Publ. Math.},
	Mrclass = {14.05},
	Mrnumber = {0163909},
	Number = {8},
	Pages = {222},
	Title = {{\'E}l{\'e}ments de g{\'e}om{\'e}trie alg{\'e}brique. {II}. {\'E}tude globale {\'e}l{\'e}mentaire de quelques classes de morphismes},
	Url = {http://www.numdam.org/item?id=PMIHES_1961__8__5_0},
	Year = {1961},
	Bdsk-Url-1 = {http://mathscinet.ams.org/mathscinet-getitem?mr=0163909}}

@article{MR0163910,
	shorthand = {EGA3I},
	Author = {Grothendieck, A. and Dieudonn{\'e}, J. A.},
	Date-Added = {2018-03-24 22:13:26 +0000},
	Date-Modified = {2018-03-24 22:13:26 +0000},
	Fjournal = {Institut des Hautes {\'E}tudes Scientifiques. Publications Math{\'e}matiques},
	Issn = {0073-8301},
	Journal = {Inst. Hautes {\'E}tudes Sci. Publ. Math.},
	Mrclass = {14.05},
	Mrnumber = {0163910},
	Number = {11},
	Pages = {167},
	Title = {{\'E}l{\'e}ments de g{\'e}om{\'e}trie alg{\'e}brique. {III}. {\'E}tude cohomologique des faisceaux coh{\'e}rents, Premi{\`e}r partie},
	Url = {http://www.numdam.org/item?id=PMIHES_1961__11__5_0},
	Year = {1961},
	Bdsk-Url-1 = {http://mathscinet.ams.org/mathscinet-getitem?mr=0163910}}
	
@article{MR0163911,
	shorthand = {EGA3II},
	Author = {Grothendieck, A. and Dieudonn{\'e}, J. A.},
	Date-Added = {2018-03-24 22:13:28 +0000},
	Date-Modified = {2018-03-24 22:13:28 +0000},
	Fjournal = {Institut des Hautes {\'E}tudes Scientifiques. Publications Math{\'e}matiques},
	Issn = {0073-8301},
	Journal = {Inst. Hautes {\'E}tudes Sci. Publ. Math.},
	Mrclass = {14.05},
	Mrnumber = {0163911},
	Mrreviewer = {H. Hironaka},
	Number = {17},
	Pages = {91},
	Title = {{\'E}l{\'e}ments de g{\'e}om{\'e}trie alg{\'e}brique. {III}. {\'E}tude cohomologique des faisceaux coh{\'e}rents, Seconde partie},
	Url = {http://www.numdam.org/item?id=PMIHES_1963__17__5_0},
	Year = {1963},
	Bdsk-Url-1 = {http://mathscinet.ams.org/mathscinet-getitem?mr=0163911}}

@article{MR0173675,
	shorthand = {EGA4I},
	Author = {Grothendieck, A. and Dieudonn{\'e}, J. A.},
	Date-Added = {2018-03-24 22:13:15 +0000},
	Date-Modified = {2018-04-23 14:28:33 +0000},
	Fjournal = {Institut des Hautes {\'E}tudes Scientifiques. Publications Math{\'e}matiques},
	Issn = {0073-8301},
	Journal = {Inst. Hautes {\'E}tudes Sci. Publ. Math.},
	Mrclass = {14.05 (13.10)},
	Mrnumber = {0173675},
	Mrreviewer = {H. Hironaka},
	Number = {20},
	Pages = {259},
	Title = {{{\'E}l{\'e}ments de G{\'e}om{\'e}trie Alg{\'e}brique. {IV}. {\'E}tude locale des sch{\'e}mas et des morphismes de sch{\'e}mas, Premi{\`e}r Partie}},
	Url = {http://www.numdam.org/item?id=PMIHES_1964__20__5_0},
	Year = {1964},
	Bdsk-Url-1 = {http://mathscinet.ams.org/mathscinet-getitem?mr=0173675}}

@article{MR0199181,
	shorthand = {EGA4II},
	Author = {Grothendieck, A. and Dieudonn{\'e}, J. A.},
	Date-Added = {2018-03-24 22:13:12 +0000},
	Date-Modified = {2018-04-23 14:29:48 +0000},
	Fjournal = {Institut des Hautes {\'E}tudes Scientifiques. Publications Math{\'e}matiques},
	Issn = {0073-8301},
	Journal = {Inst. Hautes {\'E}tudes Sci. Publ. Math.},
	Mrclass = {14.00},
	Mrnumber = {0199181},
	Mrreviewer = {H. Hironaka},
	Number = {24},
	Pages = {231},
	Title = {{\'E}l{\'e}ments de G{\'e}om{\'e}trie Alg{\'e}brique. {IV}. {\'E}tude locale des sch{\'e}mas et des morphismes de sch{\'e}mas, Seconde Partie},
	Url = {http://www.numdam.org/item?id=PMIHES_1965__24__5_0},
	Year = {1965},
	Bdsk-Url-1 = {http://mathscinet.ams.org/mathscinet-getitem?mr=0199181}}

@article{MR0217086,
	shorthand = {EGA4III},
	Author = {Grothendieck, A. and Dieudonn{\'e}, J. A.},
	Date-Added = {2018-03-24 22:13:11 +0000},
	Date-Modified = {2018-04-23 14:29:21 +0000},
	Fjournal = {Institut des Hautes {\'E}tudes Scientifiques. Publications Math{\'e}matiques},
	Issn = {0073-8301},
	Journal = {Inst. Hautes {\'E}tudes Sci. Publ. Math.},
	Mrclass = {14.55},
	Mrreviewer = {J. P. Murre},
	Number = {28},
	Pages = {255},
	Title = {{{\'E}l{\'e}ments de g{\'e}om{\'e}trie alg{\'e}brique. {IV}. {\'E}tude locale des sch{\'e}mas et des morphismes de sch{\'e}mas, Troisi{\'e}m Partie}},
	Url = {http://www.numdam.org/item?id=PMIHES_1966__28__5_0},
	Year = {1966},
	Bdsk-Url-1 = {http://mathscinet.ams.org/mathscinet-getitem?mr=0217086}}

@article{MR0238860,
	shorthand = {EGA4IV},
	Author = {Grothendieck, A. and Dieudonn{\'e}, J. A.},
	Date-Added = {2018-03-24 22:13:11 +0000},
	Date-Modified = {2018-03-24 22:14:02 +0000},
	Fjournal = {Institut des Hautes {\'E}tudes Scientifiques. Publications Math{\'e}matiques},
	Issn = {0073-8301},
	Journal = {Inst. Hautes {\'E}tudes Sci. Publ. Math.},
	Mrclass = {14.55},
	Mrreviewer = {J. P. Murre},
	Number = {32},
	Pages = {361},
	Title = {{\'E}l{\'e}ments de g{\'e}om{\'e}trie alg{\'e}brique. {IV}. {\'E}tude locale des sch{\'e}mas et des morphismes de sch{\'e}mas, Quatri{\'e}m Partie},
	Url = {http://www.numdam.org/item?id=PMIHES_1967__32__5_0},
	Year = {1967},
	Bdsk-Url-1 = {http://mathscinet.ams.org/mathscinet-getitem?mr=0238860}}

@book {FGA,
	shorthand = {FGA},
    Author = {{Fantechi}, Barbara and {G\"{o}ttsche}, Lothar and {Illusie}, Luc and {Kleiman}, Steven L. and {Nitsure}, Nitin and {Vistoli}, Angelo},
    Title = {Fundamental algebraic geometry},
    Series = {Mathematical Surveys and Monographs},
    Volume = {123},
    Note = {Grothendieck's FGA explained},
	Publisher = {American Mathematical Society, Providence, RI},
    Year = {2005},
    Pages = {x+339},
    ISBN = {0-8218-3541-6},
    Mrclass = {14-06 (14A15 14D15 14F20)},
    Mrnumber = {2222646},
    Mrreviewer = {Liam O'Carroll},
    DOI = {10.1090/surv/123},
    Url = {https://doi.org/10.1090/surv/123},
}

%@article{tlr1,
%	 shorthand = {TLoR},
% 	 title={Infinitesimal local study of formal schemes},
% 	 author={Tarr{\i}o, Leovigildo Alonso and L{\'o}pez, Ana Jerem{\i}as and Rodr{\i}guez, Marta P{\'e}rez},
% 	 journal={arXiv preprint math/0504256},
% 	 year={2005},
% 	 publisher={Citeseer}
%}

@article{tlr1,
    author = {Tarr{\'i}o, Leovigildo Alonso and L{\'o}pez, Ana Jerem{\'i}as and Rodr{\'i}guez, Marta P{\'e}rez},
    year = {2007},
    month = {},
    pages = {1341-1367},
    title = {Infinitesimal Lifting and Jacobi Criterion for Smoothness on Formal Schemes},
    volume = {35},
    journal = {Communications in Algebra},
    doi = {10.1080/00927870601115823},
}

@article{tlr2,
    author = {Tarr{\i}o, Leovigildo Alonso and L{\'o}pez, Ana Jerem{\i}as and Rodr{\i}guez, Marta P{\'e}rez},
    title = {Local structure theorems for smooth maps of formal schemes},
    journal = {Journal of Pure and Applied Algebra},
    volume = {213},
    number = {7},
    pages = {1373-1398},
    year = {2009},
    issn = {0022-4049},
    doi = {https://doi.org/10.1016/j.jpaa.2008.12.006},
    url = {https://www.sciencedirect.com/science/article/pii/S0022404908002818},
}

@book{hartshorne1977algebraic,
	shorthand = {Hart1},
	title={Algebraic Geometry},
	author={Hartshorne, R.},
	isbn={9780387902449},
	lccn={lc77001177},
	series={Graduate Texts in Mathematics},
	url={https://books.google.it/books?id=3rtX9t-nnvwC},
	year={1977},
	publisher={Springer}
}

@book{hartshorne2009deformation,
	shorthand = {Hart2},
	title={Deformation Theory},
	author={Hartshorne, R.},
	isbn={9781441915955},
	lccn={2009939327},
	series={Graduate Texts in Mathematics},
	url={https://books.google.it/books?id=bwhEX01JlXkC},
	year={2009},
	publisher={Springer New York}
}

@book{hartshorne2006ample,
	shorthand = {Hart3},
	title={Ample subvarieties of algebraic varieties},
	author={Hartshorne, Robin},
	volume={156},
	year={2006},
	publisher={Springer}
}

@book{eisenbud1995commutative,
	shorthand = {Eis1},
	title={Commutative Algebra: With a View Toward Algebraic Geometry},
	author={Eisenbud, D. and Eisenbud, P.D.},
	isbn={9780387942698},
	lccn={94017351},
	series={Graduate Texts in Mathematics},
	url={https://books.google.it/books?id=Fm\_yPgZBucMC},
	year={1995},
	publisher={Springer}
}

@book{sernesi2010deformations,
	shorthand = {Ser1},
	title={Deformations of Algebraic Schemes},
	author={Sernesi, E.},
	isbn={9783642067877},
	series={Grundlehren der mathematischen Wissenschaften},
	url={https://books.google.it/books?id=nQYFkgAACAAJ},
	year={2010},
	publisher={Springer Berlin Heidelberg}
}

@book{huybrechts2016lectures,
	shorthand = {Huy1},
	title={Lectures on K3 surfaces},
	author={Huybrechts, Daniel},
	volume={158},
	year={2016},
	publisher={Cambridge University Press}
}

@inbook{kempf_1993,
	shorthand = {Kem1},
	place={Cambridge},
	series={London Mathematical Society Lecture Note Series},
	title={Curves},
	DOI={10.1017/CBO9781107359956.008},
	booktitle={Algebraic Varieties},
	publisher={Cambridge University Press},
	author={Kempf, G.},
	year={1993},
	pages={85?97},
	collection={London Mathematical Society Lecture Note Series}
}

@article{tziolas2010smoothings,
	shorthand = {Tzi1},
	title={Smoothings of schemes with nonisolated singularities},
	author={Tziolas, Nikolaos},
	journal={Michigan Mathematical Journal},
	volume={59},
	number={1},
	pages={25--84},
	year={2010},
	publisher={University of Michigan, Department of Mathematics}
}

@book{fulton1984intersection,
	shorthand = {Ful1},
	title={Intersection Theory: },
	author={Fulton, W.},
	isbn={9783540121763},
	lccn={83016762},
	series={Ergebnisse der Mathematik und ihrer Grenzgebiete : a series of modern surveys in mathematics. Folge 3},
	url={https://books.google.it/books?id=cmoPAQAAMAAJ},
	year={1984},
	publisher={Springer-Verlag}
}

@book{sernesi2007deformations,
	shorthand = {Ser1},
	title={Deformations of algebraic schemes},
	author={Sernesi, Edoardo},
	volume={334},
	year={2007},
	publisher={Springer Science \& Business Media}
}

@misc{fantechi2021smoothing,
	shorthand = {FFP1},
	title={Smoothing semi-smooth Stable Godeaux surfaces}, 
	author={Barbara Fantechi and Marco Franciosi and Rita Pardini},
	year={2021},
	eprint={2105.00786},
	archivePrefix={arXiv},
	primaryClass={math.AG}
}

@article{hironaka1968formal,
	shorthand = {HiMa1},
	title={Formal functions and formal embeddings},
	author={Hironaka, Heisuke and Matsumura, Hideyuki},
	journal={Journal of the Mathematical Society of Japan},
	volume={20},
	number={1-2},
	pages={52--82},
	year={1968},
	publisher={The Mathematical Society of Japan}
}

